Accelerating Neural Architecture Search using Performance Prediction

Methods for neural network hyperparameter optimization and meta-modeling are computationally expensive due to the need to train a large number of model configurations. In this paper, we show that standard frequentist regression models can predict the final performance of partially trained model configurations using features based on network architectures, hyperparameters, and time-series validation performance data. We empirically show that our performance prediction models are much more effective than prominent Bayesian counterparts, are simpler to implement, and are faster to train. Our models can predict final performance in both visual classification and language modeling domains, are effective for predicting performance of drastically varying model architectures, and can even generalize between model classes. Using these prediction models, we also propose an early stopping method for hyperparameter optimization and meta-modeling, which obtains a speedup of a factor up to 6x in both hyperparameter optimization and meta-modeling. Finally, we empirically show that our early stopping method can be seamlessly incorporated into both reinforcement learning-based architecture selection algorithms and bandit based search methods. Through extensive experimentation, we empirically show our performance prediction models and early stopping algorithm are state-of-the-art in terms of prediction accuracy and speedup achieved while still identifying the optimal model configurations.

==> S_background.tex <==
\section{Background}
We experiment with our early stopping algorithm by integrating it with both a meta-modeling and hyperparameter optimization algorithm, namely MetaQNN~\citep{baker2016designing} and Hyperband~\citep{li2016hyperband}. Below we give a brief background on MetaQNN and Hyperband.

\vspace{-5pt}
\subsection{MetaQNN} 
\vspace{-5pt}

Baker et al.~\citep{baker2016designing} train a $Q$-learning~\citep{watkins1989learning} agent to design convolutional neural networks. In this method, the agent samples architectures from a large, finite space by traversing a path from input to termination layer through nodes that are different layer types. The neural network model defined by the agent's trajectory is trained on the task and its validation accuracy is presented as reward to the agent. Using an $\epsilon$-greedy exploration strategy~\citep{vermorel2005multi} and experience replay~\citep{lin1992self}, the agent becomes better with time at discovering designs that obtain high performance on the learning task. 

However, the MetaQNN method uses 100 GPU-days to train 2700 neural architectures and the similar experiment by~\cite{zoph2016neural} utilized 10,000 GPU-days to train 12,800 models on CIFAR-10. The amount of computing resources required for these approaches makes them prohibitively expensive for large datasets (e.g., Imagenet) and larger search spaces. The main computational expense of reinforcement learning-based meta-modeling methods is training the neural net configuration to $T$ epochs (where $T$ is typically a large number at which the network stabilizes to peak accuracy). $y_T$, the network accuracy at epoch $T$ is presented as reward to the learning agent.

\subsection{Hyperband}
\vspace{-5pt}
Recently,~\cite{li2016hyperband} introduced Hyperband, a random search technique based on multi-armed bandits that obtains state-of-the-art performance in hyperparameter optimization in a variety of settings. The Hyperband algorithm trains a population of models with different hyperparameter configurations and iteratively discards models below a certain percentile in performance among the population until the computational budget is exhausted or satisfactory results are obtained. 

Hyperband uses a ``last seen value'' heuristic, essentially meaning it uses the last seen validation set performance to judge which models should be thrown out. While this heuristic works very well already, we show that using a predictor trained on the partially observed learning curve can be used to do even more aggressive early stopping and speedup overall performance when compared to the original Hyperband algorithm.

%The Hyperband algorithm relies on the observation that a ``better'' hyperparameter configuration tends to learn more quickly overall, and hence a model trained with this configuration should perform better the 50th percentile when trained over a very small number of iterations, in a population of models trained with different hyperparameter configurations. They use this assumption to discard models below the 50th percentile at regular intervals.  They hedge this assumption by varying number of hyperparameters selected (breadth) and corresponding durations they are trained on (depth), and repeat this process several times until satisfactory results are obtained. 

% Concretely, Hyperband starts with a computational budget $B$ and a max iteration count $R$. Let $\eta$ denote the proportion of configurations discarded at each iteration. The outer loop of this algorithm considers a total of $s_{max} = log_\eta(R)$ randomly selected sets of hyperparameter configurations. The size of the first set of hyperparameter configurations is set to $B/(s_{max}+1)$ and continues to shrink by factor of $\eta$ in each outer loop iteration. The inner loop trains the set of hyperparameter configurations for a small number of iterations and successively culls all but the top $1/\eta$ configurations. 

%Hyperband requires two inputs (1) R, the maximum amount of resource that can be allocated to a single configuration, and (2) η, an input that controls the proportion of configurations discarded in each round of SuccessiveHalving. The two inputs dictate how many different brackets are considered; specifically, smax + 1 different values for n are considered with smax = blogη (R)c. Hyperband begins with the most aggressive bracket s = smax, which sets n to maximize exploration, subject to the constraint that at least one configuration is allocated R resources. Each subsequent bracket reduces n by a factor of approximately η until the final bracket, s = 0, in which every configuration is allocated R resources (this bracket simply performs classical random search). Hence, Hyperband performs a geometric search in the average budget per configuration and removes the need to select n for a fixed budget at the cost of approximately smax + 1 times more work than running SuccessiveHalving for a single value of n. By doing so, Hyperband is able to exploit situations in which adaptive allocation works well, while protecting itself in situations where more conservative allocations are required.

% \NNnote{to be moved to experiments once stable} We run hyperband algorithm on CIFAR10, SVHN and ILSVRC12 datasets. CIFAR10 and SVHN are run on cudaconvnet and we vary initial learning rate, learning rate reduction step size, weight decay for convolutional and fully connected layers and scale and power of local response normalization layers. CIFAR10 models are trained for 375 iterations (60 epochs) and SVHN is trained for 600 iterations (12 epochs). Total of 8489 and 16582 configurations were randomly sampled for CIFAR10 and SVHN respectively.

% ILSVRC12 was considerably more challenging because of larger image size and overall size of dataset. We randomly sampled 10\% of dataset and trained it for 500 iterations comprising of 10 epochs. We use alexnet architecture and varied learning rate and learning rate reduction step size. We were able to sample and train overall 1376 hyperparameter configurations.

% \begin{table}[]
% \centering
% \caption{Range of hyperparameter settings used in Lenet Experiment.}
% \label{lenet_hp}
% \begin{tabular}{llll}
% Hyperparameter           & Scale  & Min  & Max  \\
% Learning Rate            & log    & 1e-3 & 1e-1 \\
% Batch size               & log    & 1e1  & 1e3  \\
% Layer 2 Num Kernels (k2) & linear & 10   & 60   \\
% Layer 1 Num Kernels (k1) & linear & 5    & k2  
% \end{tabular}

==> nips_2017_workshop/S_background.tex <==
\section{Background}
We experiment with our early stopping algorithm by integrating it with both a meta-modeling and hyperparameter optimization algorithm, namely MetaQNN~\citep{baker2016designing} and Hyperband~\citep{li2016hyperband}. Below we give a brief background on MetaQNN and Hyperband.

\vspace{-5pt}
\subsection{MetaQNN} 
\vspace{-5pt}

Baker et al.~\citep{baker2016designing} train a $Q$-learning~\citep{watkins1989learning} agent to design convolutional neural networks. In this method, the agent samples architectures from a large, finite space by traversing a path from input to termination layer through nodes that are different layer types. The neural network model defined by the agent's trajectory is trained on the task and its validation accuracy is presented as reward to the agent. Using an $\epsilon$-greedy exploration strategy~\citep{vermorel2005multi} and experience replay~\citep{lin1992self}, the agent becomes better with time at discovering designs that obtain high performance on the learning task. 

However, the MetaQNN method uses 100 GPU-days to train 2700 neural architectures and the similar experiment by~\cite{zoph2016neural} utilized 10,000 GPU-days to train 12,800 models on CIFAR-10. The amount of computing resources required for these approaches makes them prohibitively expensive for large datasets (e.g., Imagenet) and larger search spaces. The main computational expense of reinforcement learning-based meta-modeling methods is training the neural net configuration to $T$ epochs (where $T$ is typically a large number at which the network stabilizes to peak accuracy). $y_T$, the network accuracy at epoch $T$ is presented as reward to the learning agent.

\subsection{Hyperband}
\vspace{-5pt}
Recently,~\cite{li2016hyperband} introduced Hyperband, a random search technique based on multi-armed bandits that obtains state-of-the-art performance in hyperparameter optimization in a variety of settings. The Hyperband algorithm trains a population of models with different hyperparameter configurations and iteratively discards models below a certain percentile in performance among the population until the computational budget is exhausted or satisfactory results are obtained. 

Hyperband uses a ``last seen value'' heuristic, essentially meaning it uses the last seen validation set performance to judge which models should be thrown out. While this heuristic works very well already, we show that using a predictor trained on the partially observed learning curve can be used to do even more aggressive early stopping and speedup overall performance when compared to the original Hyperband algorithm.

%The Hyperband algorithm relies on the observation that a ``better'' hyperparameter configuration tends to learn more quickly overall, and hence a model trained with this configuration should perform better the 50th percentile when trained over a very small number of iterations, in a population of models trained with different hyperparameter configurations. They use this assumption to discard models below the 50th percentile at regular intervals.  They hedge this assumption by varying number of hyperparameters selected (breadth) and corresponding durations they are trained on (depth), and repeat this process several times until satisfactory results are obtained. 

% Concretely, Hyperband starts with a computational budget $B$ and a max iteration count $R$. Let $\eta$ denote the proportion of configurations discarded at each iteration. The outer loop of this algorithm considers a total of $s_{max} = log_\eta(R)$ randomly selected sets of hyperparameter configurations. The size of the first set of hyperparameter configurations is set to $B/(s_{max}+1)$ and continues to shrink by factor of $\eta$ in each outer loop iteration. The inner loop trains the set of hyperparameter configurations for a small number of iterations and successively culls all but the top $1/\eta$ configurations. 

%Hyperband requires two inputs (1) R, the maximum amount of resource that can be allocated to a single configuration, and (2) η, an input that controls the proportion of configurations discarded in each round of SuccessiveHalving. The two inputs dictate how many different brackets are considered; specifically, smax + 1 different values for n are considered with smax = blogη (R)c. Hyperband begins with the most aggressive bracket s = smax, which sets n to maximize exploration, subject to the constraint that at least one configuration is allocated R resources. Each subsequent bracket reduces n by a factor of approximately η until the final bracket, s = 0, in which every configuration is allocated R resources (this bracket simply performs classical random search). Hence, Hyperband performs a geometric search in the average budget per configuration and removes the need to select n for a fixed budget at the cost of approximately smax + 1 times more work than running SuccessiveHalving for a single value of n. By doing so, Hyperband is able to exploit situations in which adaptive allocation works well, while protecting itself in situations where more conservative allocations are required.

% \NNnote{to be moved to experiments once stable} We run hyperband algorithm on CIFAR10, SVHN and ILSVRC12 datasets. CIFAR10 and SVHN are run on cudaconvnet and we vary initial learning rate, learning rate reduction step size, weight decay for convolutional and fully connected layers and scale and power of local response normalization layers. CIFAR10 models are trained for 375 iterations (60 epochs) and SVHN is trained for 600 iterations (12 epochs). Total of 8489 and 16582 configurations were randomly sampled for CIFAR10 and SVHN respectively.

% ILSVRC12 was considerably more challenging because of larger image size and overall size of dataset. We randomly sampled 10\% of dataset and trained it for 500 iterations comprising of 10 epochs. We use alexnet architecture and varied learning rate and learning rate reduction step size. We were able to sample and train overall 1376 hyperparameter configurations.

% \begin{table}[]
% \centering
% \caption{Range of hyperparameter settings used in Lenet Experiment.}
% \label{lenet_hp}
% \begin{tabular}{llll}
% Hyperparameter           & Scale  & Min  & Max  \\
% Learning Rate            & log    & 1e-3 & 1e-1 \\
% Batch size               & log    & 1e1  & 1e3  \\
% Layer 2 Num Kernels (k2) & linear & 10   & 60   \\
% Layer 1 Num Kernels (k1) & linear & 5    & k2  
% \end{tabular}

==> nips_2017_workshop/S_conclusion.tex <==
\section{Conclusion}
\vspace{-5pt}
In this paper, we focus on speeding up meta-modeling methods with an early-stopping scheme that utilizes a simple neural network performance prediction model. However, our method also accelerates hyperparameter search methods (for example, our experiments show upto 2.5x speedup on Hyperband~\cite{li2016hyperband}). With the advent of large scale automated architecture search~\citep{baker2016designing, zoph2016neural,pmlr-v70-cortes17a,negrinho2017deeparchitect,zoph2017learning,brock2017smash}, methods such as ours will be vital in exploring large and complex search spaces.


==> nips_2017_workshop/S_early_stopping.tex <==
\section{Accelerating Meta-modeling with Performance Prediction}
\vspace{-5pt}
\label{sec:early_stop}
We will use the sequential regression models to speedup meta-modeling using an \textbf{early stopping scheme} to determine whether to continue training a partially trained model configuration. If we would like to sample $N$ total neural network configurations, we begin by sampling and training $n \ll N$ configurations to create a training set $\mathcal{S}$. We then train a model $f(x_f)$to predict $y_T$. Now, given the current best performance observed $y_\text{BEST}$, we would like to terminate training a new configuration $\mathbf{x'}$ given its partial learning curve $y'(t)_{\text{1--$\tau$}}$ if $f({x_f}') = \hat y_T \le y_\text{BEST}$ so as to not waste computational resources exploring a suboptimal configuration. However, in the case $f(x_f)$ has poor out-of-sample generalization, we may mistakenly terminate the optimal configuration. If we assume that our estimate can be modeled as a Gaussian perturbation of the true value $\hat y_T \sim \mathcal{N}(y_T, \sigma(\mathbf{x}, \tau))$, then we can find the probability $p(\hat y_T \le y_\text{BEST} | \sigma(\mathbf{x}, \tau)) = \Phi(y_\text{BEST}; y_T, \sigma)$, where $\Phi(\cdot; \mu, \sigma)$ is the CDF of $\mathcal{N}(\mu, \sigma)$. Note that in general the uncertainty will depend on both the configuration and $\tau$, the number of points observed  from the learning curve. Because frequentist models do not admit a natural estimate of uncertainty, we assume that $\sigma$ is independent of $\mathbf{x}$ yet still dependent on $\tau$ and estimate it via Leave One Out Cross Validation. 

Now that we can estimate the model uncertainty, given a new configuration $\mathbf{x'}$ and an observed learning curve $y'(t)_{\text{1--$\tau$}}$,  we may set our termination criteria to be $p(\hat y_T \le y_\text{BEST}) \ge \Delta$. $\Delta$ balances the trade-off between increased speedups and risk of prematurely terminating good configurations. In many cases, one may want several configurations that are close to optimal, for the purpose of ensembling. We offer two modifications in this case. First, one may relax the termination criterion to $p(\hat y_T \le y_\text{BEST} - \delta) \ge \Delta$, which will allow configurations within $\delta$ of optimal performance to complete training. One can alternatively set the criterion based on the $n^{\text{th}}$ best configuration observed, guaranteeing that with high probability the top $n$ configurations will be fully trained. 

% \subsection{Comparison to Bayesian Methods}
% \NNnote{Rewrite this part to include results}
% We compare all results against the Bayesian learning curve extrapolation methods introduced by Domhan et al.~\citep{domhan2015speeding} and Klein et al.~\citep{klein2017learning}. Moreover, we compare against the Swersky et al.~\citep{swersky2014freeze} Gaussian process-based method \BBnote{idk if we'll have that one in time}. Finally, we compare against the ``last seen value'' heuristic used by Li et al.~\citep{li2016hyperband}\NNnote{describe the heuristic}. 

% For the methods that use prior learning curves as training data, namely ours and Bayesian Neural Network (BNN) by Klein et al.\citep{klein2017learning}, we compare performance by varying the number of fully observed curves. When training the BNN, we present it with both the fully observed learning curves and the partially observed learning curves of the remaining data. Finally, for all methods we also compare performance of predicting final accuracy by varying the fraction of validation accuracy curve available for training.

\textbf{Experiment with MetaQNN:} Baker et al~\cite{baker2016designing} develop {MetaQNN}, a $Q$-learning-based method to design convolutional neural networks. 
%In this method, the agent samples architectures from a large, finite space by traversing a path from input layer to termination layer. 
%The neural network model defined by the agent's trajectory is trained on the task and its validation accuracy is presented as reward to the agent. 
%However, the MetaQNN method uses 100 GPU-days to train 2700 neural architectures and the similar experiment by~\cite{zoph2016neural} utilized 10,000 GPU-days to train 12,800 models on CIFAR-10. The amount of computing resources required for these approaches makes them prohibitively expensive for large datasets (e.g., Imagenet) and larger search spaces. 
The main computational expense of MetaQNN and other reinforcement learning-based meta-modeling methods is training the neural network configuration to $T$ epochs (where $T$ is typically a large number at which the network stabilizes to peak accuracy).
We use $\nu$-SVR (RBF) SRM to speed up MetaQNN. First, we take 1,000 random models from the MetaQNN~\citep{baker2016designing} search space. We simulate the MetaQNN algorithm by taking 10 random orderings of each set and running our early stopping algorithm. We compare against the LCE early stopping algorithm~\citep{domhan2015speeding} as a baseline, which has a similar probability threshold termination criterion. Our SRM trains off of the first 100 fully observed curves, while the LCE model trains from each individual partial curve and can begin early termination immediately. Despite this ``burn in'' time needed by an SRM, it is still able to significantly outperform the LCE model and obtains up to 6x speedup on the original method (Figure \ref{qnn_speed_up}). 
%In addition, fitting the LCE model to a learning curve takes between 1-3 minutes on a modern CPU due to expensive MCMC sampling, and  it is necessary to fit a new LCE model each time a new point on the learning curve is observed. 
%Therefore, on a full meta-modeling experiment involving thousands of neural network configurations, our method could be faster by several orders of magnitude as compared to LCE based on current implementations. 
%Thus, for an experiment on the order of that of \cite{baker2016designing} or \cite{zoph2016neural}, many days of computation time would be added as overhead to fit the LCE models when compared to our simple model.

\begin{figure}[t]
\centering
\includegraphics[width=0.9\textwidth]{simulated_qnn_speedup.pdf}
\caption{We simulate  \textbf{speedup in MetaQNN search space} with SRMs and compare against existing methods. Triangles indicate an algorithm that successfully recovered the optimal model for more than half of the 10 orderings, and X's indicate those that did not.}
\label{qnn_speed_up}
\vspace{-10pt}
\end{figure}

\begin{wrapfigure}{r}{0.45\textwidth}
%\vspace{5pt}
\centering
\includegraphics[width=0.45\textwidth]{cifar10_q_early_stopping.pdf}
\caption{A full run of \textbf{MetaQNN on CIFAR-10 with early stopping}, with $\nu$-SVR SRM with a probability threshold $\Delta = 0.99$. Light blue bars indicate the average model accuracy per decrease in $\epsilon$, which represents the shift to a more greedy policy. The cumulative best, top 5, and top 15 show that the agent continues to find better architectures.}
%\vspace{5pt}
\label{cifar10_metaqnn}
\end{wrapfigure}

%We furthermore simulate early stopping for Resnets trained on CIFAR-10. We found that only the probability threshold $\Delta = 0.99$ resulted in recovering the top model consistently. However, even with such a conservative threshold, the search was sped up by a factor of 3.4 over the baseline. While we do not have the computational resources to run the full experiment from~\cite{zoph2016neural}, our method could provide similar gains in large scale architecture searches.
%It is not enough, however, to simply simulate the speedup because meta-modeling algorithms typically use the observed performance in order to update an acquisition function to inform future sampling. 

In addition to the simulation, we perform a full run of the MetaQNN algorithm with early stopping. In the reinforcement learning setting, the performance is given to the agent as a reward, so we need to empirically verify that substituting $\hat y_T$ for $y_T$ does not cause the MetaQNN agent to converge to a subpar policy. Replicating the MetaQNN experiment on CIFAR-10 (see Figure \ref{cifar10_metaqnn}), we find that integrating early stopping with the $Q$-learning procedure does not disrupt learning and resulted in a speedup of 3.8x with $\Delta = 0.99$. The speedup is relatively low due to a conservative value of $\Delta$. After training the top models to 300 epochs, we also find that the resulting performance (just under 93\%) is on par with original results of~\cite{baker2016designing}.


==> nips_2017_workshop/S_intro.tex <==
\vspace{-15pt}
\section{Introduction}
\vspace{-5pt}
Meta-modeling methods~\citep{bergstra2013making,verbancsics2013generative,baker2016designing,zoph2016neural} aim to design neural network architectures from scratch to reduce the amount of human expertise and labor usually required. However, these methods require training a large number of neural network configurations for identifying the right network architecture---and are hence computationally expensive. For example, Zoph and Le~\cite{zoph2016neural} train 12,800 networks using 10,000 GPUdays to design a state-of-the-art CNN for the CIFAR-10 dataset. We propose to speedup meta-modeling methods by automatically predicting final neural network performance from partially-trained learning curves and early-terminating subpar model configurations. We briefly summarize related work next. 
%While there is some prior work on neural network performance prediction using Bayesian methods~\citep{domhan2015speeding,klein2017learning}, our proposed method is significantly more accurate, accessible, and efficient. 

%When sampling many different model configurations, it is likely that many subpar configurations will be explored. Humans are quite adept at recognizing and terminating suboptimal model configurations by inspecting their partial learning curves.  Our method parameterizes learning curve trajectories with simple features derived from model architectures, training hyperparameters, and early time-series measurements from the learning curve. We use these features to train a set of frequentist regression models that predicts the final validation accuracy of partially trained neural network configurations using a small training set of fully trained curves from both image classification and language modeling domains. We use these predictions and uncertainty estimates obtained from small model ensembles to construct a simple early stopping algorithm that can speedup meta-modeling methods.

%We hope that our work leads to inclusion of neural network performance prediction and early stopping in the practical neural network training pipeline. 

==> nips_2017_workshop/S_perf_pred.tex <==
\section{Neural Network Performance Prediction}
\vspace{-5pt}
\label{sec:method}
%We first describe our model for neural network performance prediction, followed by a description of the datasets used to evaluate our model, and finally present experimental results. \vspace{-5pt}
%and method for early termination of under-performing network architectures. 
% Finally, we describe our implementation for speeding up meta-modeling and hyperparameter optimization methods. 

\begin{figure}
	\centering
	\includegraphics[width=\textwidth]{learning_curves.pdf}
	\caption{\textbf{Example learning curves} showing diversity in convergence times and curve shapes.}
	\label{learning_curves}
\end{figure}

%\subsection{Modeling Learning Curves}
%\vspace{-5pt}
\textbf{Modeling Learning Curves:} Our goal is to model the validation accuracy $y_T$ of a neural network configuration $\mathbf{x} \in \mathcal{X} \subset \mathbb{R}^d$ at epoch $T \in \mathbb{Z}^+ $ using previous performance observations $y(t)$ (see~\cite{klein2017learning}). For each configuration $\mathbf{x}$ trained for $T$ epochs, we record a time-series $y(T) = y_1, y_2, \dots, y_T$ of validation accuracies. We train a population of $n$ configurations, obtaining a set $\mathcal{S}  = \{(\mathbf{x}^1, y^{1}(t)), (\mathbf{x}^2, y^{2}(t)), \ldots , (\mathbf{x}^n, y^{n}(t))\}$. 
We propose to use a set of features $u_\mathbf{x}$, derived from the neural network configuration $\mathbf{x}$, along with a subset of time-series accuracies $y(\tau) = (y_t)_{t = 1, 2, \ldots, \tau}$ (where $1\leq \tau < T$) from $\mathcal{S}$ to train a regression model for estimating $y_T$. Our model predicts $y_T$ of a neural network configuration using a feature set $x_f = \{u_\mathbf{x}, y(t)_{\text{1--$\tau$}}\}$. For clarity, we train $T-1$ \textit{sequential regression models} (SRM), where each successive model uses one more point of the time-series validation data. 
%As we shall see in subsequent sections, this use of  is more computationally and more precise than methods that train a single Bayesian model. 
%{We experiment with several standard frequentist methods to  train a model for $y_T$, including RBF-OLS, $\nu$-Support Vector Regression ($\nu$-SVR) with linear and RBF kernels, and random forests.} 

\textbf{Features:} We use features based on time-series (TS) validation accuracies, architecture parameters (AP), and hyperparameters (HP). (1) TS: These include the validation accuracies $y(t)_{\text{1--$\tau$}} = (y_t)_{t = 1, 2, \ldots, \tau}$ (where $1\leq \tau < T$), the first-order differences of validation accuracies (i.e., ${y_t}' = (y_t - y_{t-1})$), and the second-order differences of validation accuracies (i.e., ${y_t}'' = ({y_t}' - {y_{t-1}')}$). (2) AP: These include total number of weights and number of layers. (3) HP: These include all hyperparameters used for training the neural networks, e.g., initial learning rate (full list in Appendix).

\subsection{Datasets and Training Procedures}
\vspace{-7pt}
%We now describe the datasets and training procedures used in our experiments. %We generate learning curves from randomly sampled models in four different hyperparameter search spaces. 
%We experiment with small and very deep CNNs (e.g., Resnet, Cuda-Convnet) trained on image classification datasets and with LSTMs trained with Penn Treebank (PTB), a language modeling dataset. Figure \ref{learning_curves} shows example learning curves from three of the datasets considered in our experiments. We provide brief summary of the datasets below. 
We experiment with very deep CNNs (e.g., Resnet) trained on image classification datasets and with LSTMs trained with Penn Treebank (PTB) (details in Appendix Section \ref{appendix:search_space}). 

\textbf{Deep Resnets (TinyImageNet):} We sample 500 Resnet architectures with varying depths (between 14--110), filter sizes and number of convolutional filter block outputs and train them on the TinyImageNet\footnote{https://tiny-imagenet.herokuapp.com/} dataset (200 classes with 500 $32\times32$-size train images) for 140 epochs. 

%\textbf{Deep Resnets (CIFAR-10):} We sample 500 39-layer Resnet architectures from a search space similar to~\cite{zoph2016neural}, varying kernel width, kernel height, and number of kernels. We train these models for 50 epochs on CIFAR-10.  
\textbf{MetaQNN CNNs (CIFAR-10 and SVHN):} We sample 1,000 architectures from the MetaQNN~\cite{baker2016designing} search space, varying the numbers and orderings of convolution, pooling, and fully connected layers. The model depths are 1--12 layers (SVHN) or 1--18 (CIFAR-10). Models are trained for 20 epochs.

\textbf{LSTM (PTB):} We train 300 LSTM models on the Penn Treebank dataset for 60 epochs, evaluating validation perplexity. The number of LSTM cells and hidden layer inputs vary between 10-1400.  

%\textbf{Datasets with Varying Hyperparameters:}
%\textbf{Cuda-Convnet (CIFAR-10 and SVHN):} We train Cuda-Convnet architecture~\citep{cudaconv} with varying values of initial learning rate, learning rate reduction step size, weight decay for convolutional and fully connected layers, and scale and power of local response normalization layers. We train models with CIFAR-10 for 60 epochs and with SVHN for 12 epochs.

\subsection{Prediction Performance}
\vspace{-0.5pt}
\textbf{Choice of Regression Method:} 
%We now describe our results for performing final neural network performance. 
We train our SRMs on 100 randomly sampled neural network configurations and  compute the prediction accuracy over the rest of the dataset using the coefficient of determination $R^2$. We experiment with a few different frequentist regression models, including ordinary least squares, random forests, and $\nu$-support vector machine regression ($\nu$-SVR). $\nu$-SVR with linear or RBF kernels perform the best on most datasets, though not by a large margin. For the rest of this paper, we use $\nu$-SVR RBF unless otherwise specified (see Appendix for comparison) 
% We should describe hyperparam ranges for all methods in appendix: For all experiments, we train a $\nu$-SVR sequential regression models with random search over 1000 hyperparameter configurations from the space $C \sim$ LogUniform($10^{-5}$, 10), $\nu \sim$ Uniform(0, 1), and $\gamma \sim$ LogUniform($10^{-5}$, 10) (when using the RBF kernel).
% \begin{table}[]
% \centering
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% Dataset         			& $\nu$-SVR (RBF)       	& $\nu$-SVR (Linear) 	& Random Forest 	& OLS\\ \hline
% MetaQNN (CIFAR-10) 			& $94.22 \pm0.25$ 			& $94.44\pm0.14$ 		& $92.27\pm0.91$ 	& $93.22\pm1.1$			\\ \hline
% Resnet (TinyImageNet) 		& $85.78 \pm1.82$ 			& $91.8\pm1.1$ 			& $91.37 \pm2.18$	& $90.15\pm1.8$ 		\\ \hline
% LSTM (Penn Treebank) 		& $83.29\pm7.71$ 			& $98.59\pm0.8$ 		& $91.38\pm1.97$ 	& $89.8\pm0.16$			\\ \hline
% \end{tabular}
% %\vspace{10pt}
% \caption{\textbf{Frequentist Model Comparison:} We report the coefficient of determination $R^2$ for four standard methods. Each model is trained with 100 samples on 25\% of the learning curve. We find that $\nu$-SVR works best on average, though not by a large margin.}
% \label{tab:freq}
% \end{table}


\begin{figure}
\centering
\includegraphics[width=0.9\textwidth]{scatter_plots.pdf}
\caption{\textbf{Predicted versus true final performance} with a $\nu$-SVR (RBF) model trained with 25\% of learning curve (TS), along with architecture (AP) and hyperparameter (HP) features.}
\label{scatter}
\end{figure}


\textbf{Comparison with Existing Methods:} 
We now compare the neural network performance prediction ability of SRMs with three existing learning curve prediction methods: (1) Bayesian Neural Network (BNN)~\citep{klein2017learning}, (2) the learning curve extrapolation (LCE) method~\citep{domhan2015speeding}, and (3) the last seen value (LastSeenValue) heuristic~\citep{li2016hyperband}. 
%When training the BNN, we not only present it with the subset of fully observed learning curves but also all other partially observed learning curves from the training set. While we do not present the partially observed curves to the $\nu$-SVR SRM for training, we felt this was a fair comparison as $\nu$-SVR uses the entire partially observed learning curve during inference.  Methods (2) and (3) do not incorporate prior learning curves during training.
Figure \ref{results_by_percent} shows that in all neural network configuration spaces and across all datasets, either one or both SRMs outperform the competing methods. Since LCE~\citep{domhan2015speeding} and BNN~\citep{klein2017learning} contain basis functions for exponential learning rate decay (ELRD), instead of stepwise learning rate decay used in our datasets (which has become a common practice), we trained 630 random nets with ELRD  from the 1000 MetaQNN-CIFAR10 nets. Predicting from 25\% of the learning curve, the $R^2$ is 0.95 for $\nu$-SVR (RBF), 0.48 for LCE (with extreme outlier removal, negative without), and 0.31 for BNN. This comparison illuminates another benefit of our method: we do not require handcrafted basis functions to model new learning curve types. SRMs are also much faster to train and do inference as compared to~\citep{domhan2015speeding,klein2017learning}. 
%The LastSeenValue heuristic only becomes viable when the configurations are near convergence, and its performance is worse than an SRM for very deep models. We also find that the SRMs outperform the LCE method in all experiments, even after we remove a few extreme prediction outliers produced by LCE. Finally, while BNN outperforms the LastSeenValue and LCE methods when only a few iterations have been observed, it does worse than our proposed method. In summary, we show that our simple, frequentist SRMs outperforms existing Bayesian approaches on predicting neural network performance on modern, very deep models in computer vision and language modeling tasks. 
%Since most of our experiments perform stepwise learning rate decay; it is conceivable that the performance gap between SRMs and both LCE and BNN results from a lack of sharp jump in their basis functions. We experimented with exponential learning rate decay (ELRD), which the basis functions in LCE are designed for.  This comparison illuminates another benefit of our method: we do not require handcrafted basis functions to model new learning curve types.

\begin{figure*}[t]
\centering
\includegraphics[width=1\textwidth]{results_by_percent_nips.pdf}
\caption{\textbf{Performance prediction results} comparing against BNN~\citep{klein2017learning}, LCE~\citep{domhan2015speeding}, and a ``last seen value'' heuristic \citep{li2016hyperband}. Absent results for a model indicate that it did not achieve a positive $R^2$.}
\label{results_by_percent}
\end{figure*} 

% \textbf{Training and Inference Speed Comparison:}
% Another advantage of our regression approach is speed. SRMs are much faster to train and do inference in than proposed Bayesian methods~\citep{domhan2015speeding,klein2017learning}. On 1 core of a Intel 6700k CPU, an $\nu$-SVR (RBF) with 100 training points trains in 0.006 seconds, and each inference takes 0.00006 seconds. In comparison, the LCE code  takes 60 seconds and BNN code takes 0.024 seconds on the same hardware for each inference. 
%With this we conclude that SRMs are not only much more powerful predictors, but are also much more computationally efficient.

% \subsection{Empirical Evaluation}
% We propose to train an SVR model to predict $y_T$ and utilize it for speeding up two applications: meta-modeling and hyperparameter optimization. As will be described in the following sections, we replicate the MetaQNN \citep{baker2016designing} and Hyperband \citep{li2016hyperband} experiments and augment them with our early stopping algorithm.

% \subsubsection{Meta-modeling} 
% \vspace{-5pt}
% Meta-modeling methods have recently become popular for designing network architectures from scratch. In particular, networks designed with reinforcement learning-based approaches~\citep{baker2016designing,zoph2016neural} have obtained state-of-the-art results on small image and text classification datasets. However, these methods currently require extreme computing resources. For illustration, Zoph and Le~\citep{zoph2016neural} utilized 10,000 GPU-days to train 12,800 CNN configurations and discovered a state-of-the-art model for the CIFAR-10 dataset. The amount of computing resources required for this approach makes it prohibitively expensive for large datasets (e.g., Imagenet). 

% The main computational expense of reinforcement learning-based meta-modeling methods is training the neural net configuration to $T$ epochs (where $T$ is typically a large number at which the network stabilizes to peak accuracy). $y_T$, the network accuracy at epoch $T$ is presented as reward to the learning agent. A machine learning model that provides a prediction $\hat y_T$ for the reward, using features derived from the neural network configuration and/or time-series data on accuracies ($y(t)_{\text{1--$\tau$}}, \tau \ll T$) can be used to significantly speed up the meta-modeling algorithm. In this paper, we replicate MetaQNN~\citep{baker2016designing}---a meta-modeling method based on $Q$-learning---to demonstrate this speed-up. 

% \textbf{MetaQNN:} Baker et al.~\citep{baker2016designing} train a $Q$-learning~\citep{watkins1989learning} agent to design convolutional neural networks. In this method, the agent samples architectures from a large, finite space by traversing a path from input to termination layer through nodes that are different layer types. The neural network model defined by the agent's trajectory is trained on the task and its validation accuracy is presented as reward to the agent. Using an $\epsilon$-greedy exploration strategy~\citep{vermorel2005multi} and experience replay~\citep{lin1992self}, the agent becomes better with time at discovering designs that obtain high performance on the learning task. 

% \subsection{Hyperparameter Optimization}
% \vspace{-7pt}
% Hyperparameter optimization is an important part of the neural network training process---with random search or grid search over the hyperparameter space being the practical method of choice. Recently, Li et al.~\citep{li2016hyperband} introduced \textbf{Hyperband}, a random search technique based on multi-armed bandits that obtains state-of-the-art performance in hyperparameter optimization in a variety of settings. The Hyperband algorithm trains a population of models with different hyperparameter configurations and iteratively discards models below a certain percentile in performance among the population, until the computational budget is exhausted or satisfactory results are obtained. 

% %The Hyperband algorithm relies on the observation that a ``better'' hyperparameter configuration tends to learn more quickly overall, and hence a model trained with this configuration should perform better the 50th percentile when trained over a very small number of iterations, in a population of models trained with different hyperparameter configurations. They use this assumption to discard models below the 50th percentile at regular intervals.  They hedge this assumption by varying number of hyperparameters selected (breadth) and corresponding durations they are trained on (depth), and repeat this process several times until satisfactory results are obtained. 

% Concretely, Hyperband starts with a computational budget $B$ and a max iteration count $R$. Let $\eta$ denote the proportion of configurations discarded at each iteration. The outer loop of this algorithm considers a total of $s_{max} = log_\eta(R)$ randomly selected sets of hyperparameter configurations. The size of the first set of hyperparameter configurations is set to $B/(s_{max}+1)$ and continues to shrink by factor of $\eta$ in each outer loop iteration. The inner loop trains the set of hyperparameter configurations for a small number of iterations and successively culls all but the top $1/\eta$ configurations. 

% %Hyperband requires two inputs (1) R, the maximum amount of resource that can be allocated to a single configuration, and (2) η, an input that controls the proportion of configurations discarded in each round of SuccessiveHalving. The two inputs dictate how many different brackets are considered; specifically, smax + 1 different values for n are considered with smax = blogη (R)c. Hyperband begins with the most aggressive bracket s = smax, which sets n to maximize exploration, subject to the constraint that at least one configuration is allocated R resources. Each subsequent bracket reduces n by a factor of approximately η until the final bracket, s = 0, in which every configuration is allocated R resources (this bracket simply performs classical random search). Hence, Hyperband performs a geometric search in the average budget per configuration and removes the need to select n for a fixed budget at the cost of approximately smax + 1 times more work than running SuccessiveHalving for a single value of n. By doing so, Hyperband is able to exploit situations in which adaptive allocation works well, while protecting itself in situations where more conservative allocations are required.

% % \NNnote{to be moved to experiments once stable} We run hyperband algorithm on CIFAR-10, SVHN and ILSVRC12 datasets. CIFAR-10 and SVHN are run on cudaconvnet and we vary initial learning rate, learning rate reduction step size, weight decay for convolutional and fully connected layers and scale and power of local response normalization layers. CIFAR-10 models are trained for 375 iterations (60 epochs) and SVHN is trained for 600 iterations (12 epochs). Total of 8489 and 16582 configurations were randomly sampled for CIFAR-10 and SVHN respectively.

% % ILSVRC12 was considerably more challenging because of larger image size and overall size of dataset. We randomly sampled 10\% of dataset and trained it for 500 iterations comprising of 10 epochs. We use alexnet architecture and varied learning rate and learning rate reduction step size. We were able to sample and train overall 1376 hyperparameter configurations.


==> nips_2017_workshop/S_related.tex <==
%\subsection{Related Work}
%\vspace{-5pt}
%\label{sec:related}
\textbf{Neural Network Performance Prediction:}
Domhan et al.\cite{domhan2015speeding} introduce a weighted probabilistic model for learning curves and utilize this model for speeding up hyperparameter search in small convolutional neural networks (CNNs) and fully-connected networks (FCNs). Building on~\cite{domhan2015speeding}, Klein et al.~\cite{klein2017learning} train Bayesian neural networks for predicting unobserved learning curves using a training set of fully and partially observed learning curves. Both methods rely on Markov chain Monte Carlo (MCMC) sampling procedures and handcrafted learning curve basis functions.
% In contrast to our work, this method independently models the learning curve for each network using a set of handcrafted basis functions.  Due to these methods reliance on handcrafted basis functions and expensive Monte Carlo samplers, our method is significantly simpler, more efficient, and more accurate in a variety of settings. 
% NN -- commenting this since we just said this before, and will do comparison later. 
%We also note that ~\cite{swersky2014freeze} develop a Gaussian Process kernel for predicting individual learning curves, which they use to automatically stop and restart configurations.

\textbf{Meta-modeling:} The earliest meta-modeling approaches were based on genetic algorithms~\citep{schaffer1992combinations,stanley2002evolving,verbancsics2013generative} or Bayesian optimization~\citep{bergstra2013making,shahriari2016taking}. More recently, reinforcement learning methods have become popular. Baker et al.~\cite{baker2016designing} introduce MetaQNN, a  Q-learning-based method to designs CNNs. Zoph and Le~\cite{zoph2016neural} use policy gradients to design CNNs and recurrent cell architectures.  Several meta-modeling methods~\citep{pmlr-v70-cortes17a,negrinho2017deeparchitect,zoph2017learning,brock2017smash,suganuma2017genetic} have been proposed since the publication of~\cite{baker2016designing,zoph2016neural}.
%\textbf{Hyperparameter Optimization:} We define hyperparameter optimization as an algorithmic approach for finding optimal values of design-independent hyperparameters such as learning rate and batch size, along with a limited search through the network design space. Bayesian  hyperparameter optimization methods include those based on sequential model-based optimization (SMAC)~\citep{hutter2011sequential}, Gaussian processes (GP)~\citep{snoek2012practical}, TPE~\citep{bergstra2013making}, and neural networks~\cite{snoek2015scalable}. 
%However, random search or grid search is most commonly used in practical settings~\citep{bergstra2012random}. Recently,~\cite{li2016hyperband} introduced Hyperband, a multi-armed bandit-based efficient random search technique that outperforms state-of-the-art Bayesian optimization methods.
\vspace{-5pt}
